Accuracy and Cost Claims Do Not Survive Re-Execution in Agentic VideoQA

Agentic Video Question Answering (VideoQA) systems produce answers through adaptive reasoning and tool-use trajectories, yet standard practice evaluates each system once and estimates uncertainty only across questions. This leaves a basic question untested: would the measured method effect survive if the evaluation were run again? We show that it need not. Using Static-SAGE and Dynamic-SAGE as a controlled case study, we repeat the paired comparison twice on identical SAGE-Bench question-video pairs, holding configuration, tool library, and scoring protocol fixed. In the first execution, Dynamic-SAGE outperforms Static-SAGE by +7.33 accuracy points; in the second, the effect reverses to -4.05. Both are individually significant under paired analysis, supporting opposite conclusions. The change in the paired effect between executions is highly significant and far larger than within-execution uncertainty. The reversal is consistent across question format, modality, difficulty, and video duration, and both evaluation arms move significantly. Motivated by this failure, we introduce REPAIR (REpeated PAired Inference Reliability), a protocol that repeats the paired comparison and tests whether the method effect changes across executions, separating directional reproducibility from effect-size stability. Applied across accuracy and execution metrics, REPAIR exposes three behaviors-directional reversal, magnitude shift, and effect attenuationand shows that reductions in reasoning turns and visible tool calls do not imply reproducible reductions in primitive computation or latency. The execution-level movement is comparable to, and here larger than, median gain reported by recent agentic VideoQA systems, contextualizing its magnitude without implying those systems are unstable. Significance within a single agentic execution is insufficient evidence that a reported method effect is reproducible.

==> Makefile <==
#===============================================================================
# Kurban Intelligence Lab -- paper build
#
#   make          build main.pdf (pdflatex -> bibtex -> pdflatex x2)
#   make arxiv    arxiv-submission.tar.gz, ready to upload
#   make blind    main-blind.pdf   (double-blind: no authors, no logo, no acks)
#   make logo     regenerate every logo asset from the vector master
#   make figures  regenerate the example figure
#   make clean    remove build artefacts (keeps the PDFs)
#   make purge    remove everything generated
#===============================================================================
MAIN  := main
LATEX := pdflatex -interaction=nonstopmode -halt-on-error

.PHONY: all arxiv blind logo figures clean purge
all: $(MAIN).pdf

$(MAIN).pdf: $(MAIN).tex kurbanlab.sty affiliations.tex references.bib
	$(LATEX) $(MAIN)
	-bibtex $(MAIN)
	$(LATEX) $(MAIN)
	$(LATEX) $(MAIN)
	@echo "==> $(MAIN).pdf"

# arXiv wants the .bbl, not the .bib, and no build cruft.
arxiv: $(MAIN).pdf
	@rm -rf arxiv && mkdir -p arxiv/figures arxiv/logo
	@cp $(MAIN).tex kurbanlab.sty affiliations.tex references.bib .latexmkrc $(MAIN).bbl arxiv/
	@cp figures/*.pdf arxiv/figures/ 2>/dev/null || true
	@cp logo/kil-lockup.pdf arxiv/logo/ 2>/dev/null || true
	@cd arxiv && tar czf ../arxiv-submission.tar.gz .
	@rm -rf arxiv
	@echo "==> arxiv-submission.tar.gz  (upload this)"
	@echo "    contains: $(MAIN).tex, kurbanlab.sty, affiliations.tex, $(MAIN).bbl, figures/, logo/"
	@echo "    NOT included: *.aux, *.log. references.bib IS included: arXiv ignores it,"
	@echo "    but anyone opening this tarball in Overleaf gets a working BibTeX setup."

blind:
	@sed -E 's/\\usepackage\[([^]]*)\]\{kurbanlab\}/\\usepackage[\1, blind]{kurbanlab}/' \
	     $(MAIN).tex > $(MAIN)-blind.tex
	$(LATEX) $(MAIN)-blind
	-bibtex $(MAIN)-blind
	$(LATEX) $(MAIN)-blind
	$(LATEX) $(MAIN)-blind
	@echo "==> $(MAIN)-blind.pdf  (check it: your name should appear nowhere)"

logo:
	@cd logo && sh build-logo.sh

figures:
	@cd figures && python3 make-figure.py

clean:
	@rm -f *.aux *.log *.out *.bbl *.blg *.toc *.lof *.lot *.fls *.fdb_latexmk \
	       *.synctex.gz *.nav *.snm *.vrb $(MAIN)-blind.tex
	@echo "==> cleaned"

purge: clean
	@rm -f $(MAIN).pdf $(MAIN)-blind.pdf arxiv-submission.tar.gz
	@rm -rf arxiv

